A Concise Guide to Elicitation Methodology

One of the open questions in the field of interaction design is "what inputs or interaction techniques should be used with augmented reality devices?" The transition from a touchpad and a keyboard to a multi-touch device was relatively small. The transition from a multi-touch device to an HMD with no controllers or clear surface to interact with is more complicated. This book is a guide for how to figure out what interaction techniques and modalities people prefer when interacting with those devices. The name of the technique covered here is Elicitation. Elicitation is a form of participatory design, meaning design with direct end-user involvement. By running an elicitation study researchers can observe unconstrained human interactions with emerging technologies to help guide input design.

==> latexmkrc <==
$makeindex  = 'makeindex -s StyleInd.ist %O -o %D %S';

# support for the glossaries package:
add_cus_dep('glo', 'gls', 0, 'makeglossaries');
add_cus_dep('acn', 'acr', 0, 'makeglossaries');
sub makeglossaries {
  system("makeglossaries \"$_[0]\"");
}

# support for the nomencl package:
add_cus_dep('nlo', 'nls', 0, 'makenlo2nls');
sub makenlo2nls {
  system("makeindex -s nomencl.ist -o \"$_[0].nls\" \"$_[0].nlo\"");
}

# from the documentation for V. 2.03 of asymptote:
sub asy {return system("asy \"$_[0]\"");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

# metapost rule from http://tex.stackexchange.com/questions/37134
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}
